Data-driven Day Ahead Market Prices Forecasting: A Focus on Short Training Set Windows

This study investigates the performance of machine learning models in forecasting electricity Day-Ahead Market (DAM) prices using short historical training windows, with a focus on detecting seasonal trends and price spikes. We evaluate four models, namely LSTM with Feed Forward Error Correction (FFEC), XGBoost, LightGBM, and CatBoost, across three European energy markets (Greece, Belgium, Ireland) using feature sets derived from ENTSO-E forecast data. Training window lengths range from 7 to 90 days, allowing assessment of model adaptability under constrained data availability. Results indicate that LightGBM consistently achieves the highest forecasting accuracy and robustness, particularly with 45 and 60 day training windows, which balance temporal relevance and learning depth. Furthermore, LightGBM demonstrates superior detection of seasonal effects and peak price events compared to LSTM and other boosting models. These findings suggest that short-window training approaches, combined with boosting methods, can effectively support DAM forecasting in volatile, data-scarce environments.

==> Tables/GreekBM.tex <==
\begin{table}[!t]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Name of the procedure} & \textbf{Balancing Capacity Market} & \textbf{Balancing Energy Market} & \textbf{Imbalances Settlement Market} \\ \hline
\textbf{Time resolution}       & 30 minutes                        & 15 minutes                       & 15 minutes                            \\ \hline
\textbf{Objective}             & Balancing capacity procurement     & Balancing energy procurement      & Metering and Settlement               \\ \hline
\textbf{Ancillary services}    & FCR, aFRR, mFRR                   & aFRR, mFRR                       & -                                     \\ \hline
\textbf{Remuneration rule}     & Capacity remunerated pay-as-bid    & aFRR remunerated pay-as-bid       & Single Imbalance price                \\ 
                               &                                   & mFRR remunerated at market clearing prices & Volumes, prices and settlement amounts calculated \\ \hline
\textbf{Real time operation}   & Unit Commitment Schedule (from the ISP) & -                               & -                                     \\ \hline
\end{tabular}%
}
\caption{Overview of Greek Balancing Market (Procedures executed sequentially from left to right)}
\label{tab:GreekBM}
\end{table}

